MCAL: Minimum Cost Human-Machine Active Labeling

Today, ground-truth generation uses data sets annotated by cloud-based annotation services. These services rely on human annotation, which can be prohibitively expensive. In this paper, we consider the problem of hybrid human-machine labeling, which trains a classifier to accurately auto-label part of the data set. However, training the classifier can be expensive too. We propose an iterative approach that minimizes total overall cost by, at each step, jointly determining which samples to label using humans and which to label using the trained classifier. We validate our approach on well known public data sets such as Fashion-MNIST, CIFAR-10, CIFAR-100, and ImageNet. In some cases, our approach has 6x lower overall cost relative to human labeling the entire data set, and is always cheaper than the cheapest competing strategy.

==> 0_config.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% hyperref configuration
% \PassOptionsToPackage{usenames,dvipsnames}{color} % color is loaded by hyperref
% \hypersetup{pagebackref=true,
%             unicode=true,
%             colorlinks=true,
%             linkcolor=blue,
%             citecolor=blue,
%             anchorcolor=blue,
%             urlcolor=blue,
%             breaklinks=true,
%             bookmarks=false,
%             letterpaper=true}
            
\urlstyle{same}

%% caption configuration
%\captionsetup{margin=10pt,font=small,labelfont=bf}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% other scaling, separation configuration, do not modify
\makeatletter
\def\maxwidth{\ifdim\Gin@nat@width>\linewidth\linewidth\else\Gin@nat@width\fi}
\def\maxheight{\ifdim\Gin@nat@height>\textheight\textheight\else\Gin@nat@height\fi}
\makeatother
% Scale images if necessary, so that they will not overflow the page
% margins by default, and it is still possible to overwrite the defaults
% using explicit options in \includegraphics[width, height, ...]{}
\setkeys{Gin}{width=\maxwidth,height=\maxheight,keepaspectratio}
\setlength{\emergencystretch}{3em}  % prevent overfull lines
\providecommand{\tightlist}{%
  \setlength{\itemsep}{0pt}\setlength{\parskip}{0pt}}
\setcounter{secnumdepth}{5}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% para spacing
\makeatletter
\let\origsection\section
\let\origsubsection\subsection
\let\origparagraph\paragraph

\renewcommand\section{\@ifstar{\starsection}{\nostarsection}}
\renewcommand\subsection{\@ifstar{\starsubsection}{\nostarsubsection}}

%% Change these to control spacing for section headers/paras

\newcommand\sectionprelude{\vspace{0ex}}
\newcommand\sectionpostlude{\vspace{0ex}}
\newcommand\subsectionprelude{\vspace{0ex}}
\newcommand\subsectionpostlude{\vspace{0ex}}

\newcommand\nostarsection[1]{\sectionprelude\origsection{#1}\sectionpostlude}
\newcommand\starsection[1]{\sectionprelude\origsection*{#1}\sectionpostlude}

\newcommand\nostarsubsection[1]{\subsectionprelude\origsubsection{#1}\subsectionpostlude}
\newcommand\starsubsection[1]{\subsectionprelude\origsubsection*{#1}\subsectionpostlude}

\makeatother

\newcommand\paraspace{\vspace*{0.25ex}}
\providecommand\parab[1]{\paraspace\noindent\textbf{#1}}
\providecommand\parae[1]{\textbf{\textit{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Change these to control figure/float spacing
\setlength{\textfloatsep}{3pt plus 2.0pt minus 3.0pt}
\setlength{\abovecaptionskip}{3pt plus 2.0pt minus 3.0pt}
\setlength{\belowcaptionskip}{2pt plus 2.0pt minus 3.0pt}
\newcommand{\figwidthfrac}{0.9}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Change these to control equation spacing
\apptocmd\normalsize{%
\abovedisplayskip=5pt
\abovedisplayshortskip=5pt
\belowdisplayskip=5pt
\belowdisplayshortskip=5pt
}{}{}

%%%%%%
\hypersetup{final}
%%\DeclareMathSizes{10}{9.5}{7}{5}

\renewcommand\footnotetextcopyrightpermission[1]{} % removes footnote with conference info
\setcopyright{none}
%\setcopyright{acmcopyright}
%\setcopyright{acmlicensed}
%\setcopyright{rightsretained}
%\setcopyright{usgov}
%\setcopyright{usgovmixed}
%\setcopyright{cagov}
%\setcopyright{cagovmixed}
\settopmatter{printacmref=false, printccs=false, printfolios=true}
% DOI
\acmDOI{}
% ISBN
\acmISBN{}
%Conference
\acmConference[Submitted for review]{}
\acmYear{2021}
\copyrightyear{}
%% {} with no args suppresses printing of the price
\acmPrice{}
\pagestyle{plain}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> broader_impact.tex <==
\section*{Broader Impact}

In this paper, we introduce Min-Cost Active Labeling (\sysname), a hybrid human machine labeling system that leverages active learning to minimize groundtruth data overall acquisition cost.

Dataset labeling is often prohibitively expensive, which can limit the generalization of machine learning algorithms to a wider range of new settings and applications. While most machine learning research uses publicly available benchmarks, it is more difficult to evaluate research on more specialized settings for which there is no accurate groundtruth. By reducing the overall dataset building cost, \sysname fundamentally democratizes groundtruth acquisition.

The potential risks of a cheaper approach to larger scale dataset acquisition have not received enough attention. These include: (i) environmental damage due to more data collected and storage consumed, as well as more training cycles incurred both in the process of data collection and consumption, (ii) privacy implications due to the commoditization of data without obtaining enough consent and proper law and regulation in place, and (iii) ethical treatment of human workers used for data labeling.

We see research opportunities in applying \sysname to production systems for inventing novel capabilities not previously demonstrated. To mitigate the associated risks, we encourage research to understand the implicit impact, which is often not measured by dollar values, and to follow best practices in data privacy and pricing. Further, we also encourage  research to investigate other side effects and approaches to reduce potential negative impact while collecting datasets for a particular custom application.

==> discussion.tex <==
{\color{blue}
\section{Discussion}
\label{sec:discussion}
Instead of a constraint of labeling error, \sysname can be generalied to other constraints, such as a limited total budget. \sysname algorithm can be cast differently to search for the lowest error satisfying a given budget constraint. Specifically, with the same model for estimation of network error and total cost (\secref{sec:motivation}), instead of searching the $\sdbm$ for minimum total cost while error constraint is satisfied (line 18 of Algorithm 1), we can search for minimum estimated error while the total cost is within budget. The difference is: in the former case, we can always resort to human labeling when error constraint cannot be satisfied; in the latter case, we can only sacrifice the total accuracy by stopping the training process and taking the model's output when the money budget is too low. 
}

==> fig_latex/AL_Ablation.tex <==
\begin{figure}
  \centering
%   \includegraphics[width=\columnwidth]{fig/Motivation/ALvsNoAL_Amazon.eps}
  \includegraphics[width=\columnwidth]{fig/Motivation/ALvsNoAL_Amazon-eps-converted-to.pdf}
%   \vspace*{-0.15in}
  \captionof{figure}{Active learning gains using Amazon Labeling}
  \label{fig:ALvsNoAL-Amazon}
  \vspace{-3mm}
\end{figure}
